ShapeFlow: Dynamic Shape Interpreter for TensorFlow

We present ShapeFlow, a dynamic abstract interpreter for TensorFlow which quickly catches tensor shape incompatibility errors, one of the most common bugs in deep learning code. ShapeFlow shares the same APIs as TensorFlow but only captures and emits tensor shapes, its abstract domain. ShapeFlow constructs a custom shape computational graph, similar to the computational graph used by TensorFlow. ShapeFlow requires no code annotation or code modification by the programmer, and therefore is convenient to use. We evaluate ShapeFlow on 52 programs collected by prior empirical studies to show how fast and accurately it can catch shape incompatibility errors compared to TensorFlow. We use two baselines: a worst-case training dataset size and a more realistic dataset size. ShapeFlow detects shape incompatibility errors highly accurately -- with no false positives and a single false negative -- and highly efficiently -- with an average speed-up of 499X and 24X for the first and second baseline, respectively. We believe ShapeFlow is a practical tool that benefits machine learning developers. We will open-source ShapeFlow on GitHub to make it publicly available to both the developer and research communities.

==> background.tex <==
\section{Background}
\label{sec:background}

\subsection{Empirical studies on deep learning code bugs}
There has been a recent effort in collecting bugs that often occur in the deep learning paradigm~\cite{issta-bug-collection, fse-bug-collection}. 
The empirical studies collect programs from StackOverFlow posts and Github repositories.
These programs are written in one of the deep learning libraries like TensorFlow, Pytorch, Keras, and Caffe.
They have generated significantly large datasets containing bugs in deep-learning programs. 
Zhang et al.~\cite{issta-bug-collection} collected programs written in TensorFlow and open-sourced it after adding the corresponding fixed versions of the buggy programs. 
Johirul et al.~\cite{fse-bug-collection} collected programs written in five deep learning libraries. 
Although they did not provide the code in the programs, they listed the StackOverFlow posts and Github repositories examined.% without the code.
Both these studies have attempted to categorize the programs based on their bug types, root causes of the bugs, and their effects. 
Both these studies have concluded that shape incompatibility error or shape incompatibility error is a widespread bug faced by many deep-learning programmers. 

Other common kinds of errors in deep learning programs include the bugs due to change in API or misuse of an API by a programmer. 
Modern code editors have powerful extensions that can detect API bugs and are therefore not a target of our work. 

\subsection{TensorFlow}
TensorFlow is a declarative programming framework, which means that rather than executing code immediately, it builds a computational graph consisting of \textit{operation} nodes, which are created by the programmer's code.
The computational graphs are build statically before a model can train. 
This is the core difference between TensorFlow and Pytorch; Pytorch is dynamic and imperative.
Computational graphs can leverage the highly efficient C++ and CUDA~\cite{cuda-paper} (computing platform to accelerate deep learning) integration for better performance.% (faster training and inference).
Since during the graph construction phase, concrete values for input data shape and several other architectural layers are unknown, a special construct called ``placeholders'' allows programmers to declare nodes in the computational graph with unresolved shape.
An episode of execution of code in the Tensorflow library is called a session.
When the `session.run' function is called, the minimum connected subgraph of the computational graph is executed to run the operations listed in the particular `session' object.
The input to each operation is a tensor, and the output is another tensor. 
The ``placeholders'' in a session's subgraph must be populated before calling `session.run' function on it.

